Fairness Scheduling in User-Centric Cell-Free Massive MIMO Wireless Networks

We consider a user-centric cell-free massive MIMO wireless network with $L$ remote radio units, each with $M$ antennas, serving $K_{\rm tot}$ user equipments (UEs). Most of the literature considers the regime $LM \gg K_{\rm tot}$, where the $K$ UEs are active on each time-frequency slot, and evaluates the system performance in terms of ergodic rates. In this paper, we take a quite different viewpoint. We observe that the regime of $LM \gg K_{\rm tot}$ corresponds to a lightly loaded system with low sum spectral efficiency (SE). In contrast, in most relevant scenarios, the number of UEs is much larger than the total number of antennas, but users are not all active at the same time. To achieve high sum SE and handle $K_{\rm tot} \gg ML$, users must be scheduled over the time-frequency resource. The number of active users $K_{\rm act} \leq K_{\rm tot}$ must be chosen such that: 1) the network operates close to its maximum SE; 2) the active user set must be chosen dynamically over time in order to enforce fairness in terms of per-user time-averaged throughput rates. The fairness scheduling problem is formulated as the maximization of a concave componentwise non-decreasing network utility function of the per-user rates. Intermittent user activity imposes slot-by-slot coding/decoding which prevents the achievability of ergodic rates. Hence, we model the per-slot service rates using information outage probability. To obtain a tractable problem, we make a decoupling assumption on the CDF of the instantaneous mutual information seen at each UE $k$ receiver. We approximately enforce this condition with a conflict graph that prevents the simultaneous scheduling of users with large pilot contamination and propose an adaptive scheme for instantaneous service rate scheduling. Overall, the proposed dynamic scheduling is robust to system model uncertainties and can be easily implemented in practice.

==> 01_abstract.tex <==
%!TEX root = scheduling-journal.tex

\begin{abstract}
	We consider a user-centric scalable cell-free massive MIMO network with $L$ distributed remote radio units, each with $M$ antennas, serving $\Ktot$ user equipments (UEs). Many works in the current literature assume $LM$ much larger than $\Ktot$, consider all $\Ktot$ UEs to be active simultaneously and evaluate the system performance in terms of ergodic rates. In this user density regime, large user rates are achieved but the system does not operate at its full capability, i.e., it is far away from reaching the maximum possible sum rate. 
	In addition, cell-free massive MIMO is envisaged for high user density scenarios, where $\Ktot$ is much larger than $LM$. Of course, in this regime it does not make sense to serve all UEs simultaneously on each time-frequency-slot, requiring some form of user scheduling.
%	We investigate the user density regime, in which the network operates at full load, i.e., adding more UEs to the network and continue serving all UEs simultaneously would not lead to a significant increase of the system performance.
	We thus investigate scheduling approaches such that on each slot the number of simultaneously active UEs $\Kact < \Ktot$ is approximately optimal in the sense that 1) the network operates at full load and 2) each scheduled UE is served with a relative large data rate.
	Furthermore, with dynamic scheduling, the usual metric of ``ergodic rate'' used in most current cell-free massive MIMO literature becomes meaningless, since it is impossible to transmit long codewords over a large number of time-frequency slots. Instead, the ``instantaneous'' rate must be allocated according to an information outage probability criterion, i.e., a user is served with an allocated rate only if the instantaneous mutual information is larger than the allocated rate. The performance metric of interest is thus the user throughput rate as an average data rate over slots.
	A framework using virtual arrival processes and queues is used to impose throughput fairness among all users via a scheduler designed to maximize a suitably defined concave componentwise non-decreasing network utility function of the user throughput rates.
	Two different approaches for the joint assignment of uplink pilots for channel estimation and formation of user-centric RU clusters are investigated, differing in the required level of cooperation between UEs and network infrastructure nodes.
	The simulations address uplink and downlink transmission, and show that the proposed scheduling approaches can increase fairness among users compared to random, round-robin and max-sum-rate scheduling. Depending on the utility function, a desired distribution of the users' long-term average data rate can be achieved. The schedulers are implemented in a centralized and a {\em scalable} distributed way, where the results show that the system performance difference between the two implementations is negligible. 
	We also provide results for coding over a single time-frequency slot or a limited number $F$ of slots, modeling ``wideband transmission''. This provides an insight into the benefit of the limited amount of frequency diversity that can be achieved in practical systems. 
\end{abstract}

\begin{IEEEkeywords}
	User-centric, cell-free massive MIMO, fairness, scheduling, user density.
\end{IEEEkeywords}

==> bio_Issei_Kanno.tex <==

{Issei Kanno}
received a Ph.D. degree from Tokyo Institute of Technology, Tokyo, Japan, in 2008.

He then joined KDDI Corporation, where he has been engaged in research on software defined radio, antennas, and propagation in mobile communication systems. From 2013 to 2015, he was engaged in research on cognitive radio with Advanced Telecommunication Research Institute International (ATR). Since 2015, he has been engaged in research on wireless communication systems including 5G and beyond at KDDI Research Inc. His current research interests include signal processing and resource utilization for wireless communication systems.

Dr. Kanno received the Best Paper Award at IEEE WCNC 2010 from IEEE, the Young Researcher's Award, and the Distinguished Service Award from IEICE in 2012.

==> bio_Noboru_osawa.tex <==

{Noboru Osawa}
received a B.E. and M.E. degrees and Ph.D. in communication engineering from Osaka University, Osaka, Japan, in 2014, 2016 and 2019.
He is currently a research engineer in KDDI research Inc., Japan.
He has been engaged in research and development on wireless communication systems and wireless signal processing.

==> bio_Takeo_ohseki.tex <==

{Takeo Ohseki}  (M '95)
received B.E. and M.E. degrees in electrical and electronics engineering from the Tokyo Institute of Technology, Tokyo, Japan, in 1997 and 1999 respectively. In 1999, he joined KDDI Corp. and has been engaged in research and development on wireless access and mobile communications systems. He has also been involved in the standardization work in 3GPP RAN working group 1 for many years, and received ITU-AJ Encouragement Awards in 2021. He is currently an Expert with the Wireless Communications System Laboratory, KDDI Research, Inc.


==> bio_caire_ieee.tex <==

{Giuseppe Caire } (S '92 -- M '94 -- SM '03 -- F '05) 
was born in Torino in 1965. He received a
B.Sc. in Electrical Engineering  from Politecnico di Torino in 1990, 
an M.Sc. in Electrical Engineering from Princeton University in 1992, and a Ph.D. from Politecnico di Torino in 1994. 
He has been a post-doctoral research fellow with the European Space Agency (ESTEC, Noordwijk, The Netherlands) in 1994-1995,
Assistant Professor in Telecommunications at the Politecnico di Torino, Associate Professor at the University of Parma, Italy, 
Professor with the Department of Mobile Communications at the Eurecom Institute,  Sophia-Antipolis, France,
a Professor of Electrical Engineering with the Viterbi School of Engineering, University of Southern California, Los Angeles,
and he is currently an Alexander von Humboldt Professor with the Faculty of Electrical Engineering and Computer Science at the Technical University of Berlin, Germany.

He received the Jack Neubauer Best System Paper Award from the IEEE Vehicular Technology Society in 2003,  the
IEEE Communications Society and Information Theory Society Joint Paper Award in 2004 and in 2011, 
the Okawa Research Award in 2006,   
the Alexander von Humboldt Professorship in 2014, the Vodafone Innovation Prize in 2015, an ERC Advanced Grant in 2018, 
the Leonard G. Abraham Prize for best IEEE JSAC paper in 2019, the IEEE Communications Society Edwin Howard Armstrong Achievement Award in 2020, the 2021 Leibniz Prize  of the German National Science Foundation (DFG), and the 
CTTC Technical Achievement Award of the IEEE Communications Society in 2023.  Giuseppe Caire is a Fellow of IEEE since 2005.  He has served in the Board of Governors of the IEEE Information Theory Society from 2004 to 2007,
and as officer from 2008 to 2013. He was President of the IEEE Information Theory Society in 2011. 
His main research interests are in the field of communications theory, information theory, channel and source coding
with particular focus on wireless communications.   


==> bio_goettsch_ieee.tex <==

{Fabian G\"ottsch} (SM' 22)
received his B.Eng. in Industrial Engineering from Kiel University of Applied Sciences in 2016 and his M.Sc. degree in Electrical Engineering in 2020 from the Technical University of Berlin. From 2016 to 2019, he was with the Fraunhofer Heinrich Hertz Institute in the Signal and Information Processing Group. From 2019 to 2020, he participated in an internship at the National Institute of Informatics, Tokyo, in the Information Systems Architecture Science Research Division. From 2020 to 2021, he was with the Vodafone Chair for Mobile Communications Systems at the Technical University of Dresden. Since March 2021, he is pursuing a Ph.D. at the Communications and Information Theory Chair at the Technical University of Berlin. 
